Seamless Variability Management With the Virtual Platform

Customization is a general trend in software engineering, demanding systems that support variable stakeholder requirements. Two opposing strategies are commonly used to create variants: software clone & own and software configuration with an integrated platform. Organizations often start with the former, which is cheap, agile, and supports quick innovation, but does not scale. The latter scales by establishing an integrated platform that shares software assets between variants, but requires high up-front investments or risky migration processes. So, could we have a method that allows an easy transition or even combine the benefits of both strategies? We propose a method and tool that supports a truly incremental development of variant-rich systems, exploiting a spectrum between both opposing strategies. We design, formalize, and prototype the variability-management framework virtual platform. It bridges clone & own and platform-oriented development. Relying on programming-language-independent conceptual structures representing software assets, it offers operators for engineering and evolving a system, comprising: traditional, asset-oriented operators and novel, feature-oriented operators for incrementally adopting concepts of an integrated platform. The operators record meta-data that is exploited by other operators to support the transition. Among others, they eliminate expensive feature-location effort or the need to trace clones. Our evaluation simulates the evolution of a real-world, clone-based system, measuring its costs and benefits.

==> Discussion.tex <==

\section{Discussion}\label{sec:discussion}
\noindent
\tb{moved to prev. section}
A significant aspect of the framework is that there is no overhead for performing the asset-oriented operators. Asset-oriented operators are already invoked by the developers, so the cost of adding a file or a class or a method is none. The tool can be played as a light-weight background application that silently listens and records the events occurring in real time. The feature-oriented operators also take minimal amount of effort. In fact, Ji \textit{et al.}\,\cite{ji2015maintaining} show that the average cost of annotating one feature using the annotation syntax presented in Clafer takes an average of 1.5 lines. The same paper discusses that the average time for finding a feature manually in a source code repository is 15 minutes. Moreover, the lazy strategy of locating features requires the knowledge of the project, a strong reliance on the developers' memory, and an understanding of how implementation can be scattered in terms of cross-cutting features.

\tb{moved to prev. section}
Our analysis of the results of application of our framework on the case study of Clafer Web Tools shows promising results in terms of saved effort and time. By simulating the development of the case study with feature-oriented information, we are able to save as high as 82\

We allow feature models to be a part of assets of any type and level because software projects can include components not developed by the internal team. Having a feature model as part of assets in the lower level of the hierarchy than the repository asset provides a feature-oriented perspective to the software. They also prevent the feature models belonging to the higher level assets to not grow drastically or include very fine-grained features. While mapping the assets to features, we also enforce the condition that the feature being mapped belongs to the feature model of the closest ancestors. That way, if an asset is being mapped to a feature not present in the feature model of the closest ancestor having a feature model, we notify the developers about the missing feature. She can then decide to add the feature or correct the mistake, if any. 

While we implement a stand-alone tool for our framework, it is important to note that it can be applied in a number of ways. For example, the light-weight structures and feature-operators can be added as an extension to Git, which already caters for a number of asset-oriented operators (\addasset,\removeasset,\changeasset). In addition, simplistic storage mechanisms like text files or databases can be plugged into the framework to keep a log of clone and propagate history over time. We use data simplistic structures to store trace information on the fly for performance reasons, but an integration with a storage medium is easy and likely.



%Can also be described as limitation of state into the art in section 3.}\tb{yes, we should state that earlier in the section when saying that we can support the calculator scenario}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> activities.tex <==

\section{Development Activities}\label{sec:activities}\label{sec:clonemgmtactivities}
\looseness=-1
We extracted activities supported by techniques for supporting \co (a.k.a., clone management), or the migration of cloned variants to an integrated platform (a.k.a., product-line migration).
From our expert knowledge, we identified five relevant works on clone management and product-line migration. The product-line migration framework by 
Rubin et al.\,\cite{rubin.ea:2013:framework,Rubin2015} comprises a set of operators that support the narrative that a mechanization---i.e., an operator-based perspective---leads to more efficient implementation and support. The framework and tool ECCO Fischer et al.\,\cite{fischer.ea:2014:ecco} relies on heuristics to identify commonalities and allows composing new product variants using reusable assets. The tool BUT4Reuse by Martinez et al.\,\cite{MartinezBut4Reuse} is an extraction-based technique for product-line migration, including support for feature-model synthesis. The tool VariantSync by Pfofe et al.\,\cite{variantsync:2016} supports clone-management by easing the synchronization of assets among cloned variants. The operators and branching models for clone management in version-control systems by Montalvillo and D{\'\i}az\,\cite{montalvillo2015tuning} allow isolated variant development with change propagation, but without using the notion of features, as opposed to the other frameworks.
More details about these works are in our online appendix\,\cite{appendix:online}, including a description of their differences to the virtual platform.



We identified the following activities supported by the frameworks, at different levels of automation. These provided a baseline to specify and formalize the virtual platform operators.








\looseness=-1
\parhead{Feature Identification} determines the features that are implemented or defined in a variant or assets.
We found different mechanisms for feature identification, some of which require additional assets as input\,\cite{Rubin2015} (e.g., requirements documents or issue-tracker data), or leave it to the user to specify the list of features\,\cite{fischer.ea:2014:ecco,MartinezBut4Reuse,variantsync:2016}. 

\looseness=-1
\parhead{Feature Location} recovers the traceability between a feature and the assets implementing or defining it (i.e., the feature location). A feature can be embedded in source code, mapped to a file or a folder, or entailed in a requirements document.
When performed manually, feature location is an involved and error-prone task\,\cite{wang.ea:2013:howfeaturelocationdone,krueger2018featurelocation}.
A great variety of automated techniques is available\,\cite{Rubin2013}, all with different assumptions and capabilities; however, on realistic codebases, they usually fall short in terms of either precision or recall.


\looseness=-1
\parhead{Feature Dependency Management} supports declaring and maintaining constraints among features, ranging from binary dependencies (e.g., \textit{requires}) to propositional expressions over features. 
The frameworks supporting it rely on feature models for it, taken into account by other activities of the respective frameworks.





 

\looseness=-1
\parhead{Feature Modeling} is about creating and evolving a feature model---an intuitive, tree-like structure of features together with feature constraints.
A feature model offers various benefits, for example, it allows developers keeping an oveview understanding of the system, communicating with non-technical stakeholders, and configuring a concrete variant using an interactive configurator tool.

 


\looseness=-1
\parhead{Storing Feature-to-Asset Mappings} is relevant to maintain the locations of features in the assets. Developers use the mapping to evolve and maintain features, e.g., remove or clone them.
Such mappings are crucial for clone management with features, to avoid expensive feature location effort\,\cite{wang.ea:2013:howfeaturelocationdone,krueger2018featurelocation}.

\looseness=-1
\parhead{Clone Detection} identifies cloned assets in a set of variants.
A well-established taxonomy \cite{roy2007survey} distinguishes four clones types, the first three of which are particularly relevant for our \co scenario:
\textit{identical parts}, \textit{almost-identical parts} (except for naming), \textit{similar parts} (identical modulo minor changes), and \textit{re-implementations} of the same functionality.
A large tool landscape of clone detectors is available and can support frameworks during clone management; however, these tools often have scalability vs. accuracy trade-offs.

\looseness=-1
\parhead{Change Propagation} (semi-)automatically propagates changes (e.g., bug fixes, refactorings, behavior changes) among variants.
When performed completely manually, it involves a large effort to locate the propagation targets (possibly in several variants) and replicate the changes from the source.


\looseness=-1
\parhead{Creation of Reusable Assets} produces assets that can be used to derive variants. 
Such assets are usually equipped with a variability mechanism---an implementation technique for variation points, typically classified into annotational mechanisms (as we rely on, see \secref{sec:structures}), such as the C preprocessor or into compositional techniques, such as feature modules or component frameworks\,\cite{behringer.ea:2017:peopl,kaestner.ea:2008:cide}.




\longv{\myparhead{Product Derivation} refers to the ability to derive a partial or complete product from a given configuration, that is, a valid selection of features.
A clone management framework may rely on the derivation method from the included variability mechanism:
In compositional mechanisms, assets are assembled from smaller building blocks; when using annotational mechanisms, certain annotated parts of an asset are removed to produce the assets of a variant \cite{kaestner.ea:2008:cide}.}


\parhead{Variant Integration} differs from software merging by taking variability into account, and in our case, it is
important to consider the features the variants map to.
Integration conflicts may be resolved manually or using tool support, which might require domain knowledge and involve low-level code edits\,\cite{lillack2019incline}.
 

\parhead{Variant Comparison} compares assets to find commonalities and variabilities. Similar to clone detection, variant comparison can be useful in feature identification and feature location. 






==> backgroundrelatedwork.tex <==

\section{Background and Related Work}\label{sec:backgroundrelatedwork}

In this section,\longv{first, we introduce the general background on variability management in systems developed using \co.
Second,} we discuss the most closely related previous works, which either aim to support the independent development of several cloned variants (clone management), or the integration of variants to a product line platform (variant integration). We synthesize a set of common activities from these works, and perform a comparative analysis of the state-of-the-art works against Virtual Platform. Finally, we discuss additional related work.

\tb{actually should add the original VP paper here \cite{antkiewicz2014flexible}}

\longv{\subsection{Managing Variability in Systems Developed using Clone\,\&\,Own}
\looseness=-1
The research on variant-rich systems has usually focused on engineering software product lines\,\cite{clements.ea:01:software,czarnecki.ea:00:generative,linden.ea:2007:practices,apel.ea:2013:fospl}---portfolios of systems in a particular domain. Software product line engineering (SPLE) is a strategy that systematically exploits the commonalities and manages the variabilities among the variants. It comprises two main processes. In domain engineering, a platform with shared assets (e.g., code, requirements, test cases) is created. This platform uses various variability-implementation techniques. In application engineering, new variants are derived by binding these variabilities, where each variant constitutes one particular platform configuration.


In industrial practice, however, \co is still the preferred strategy, given its simplicity, flexibility, and provided independence\,\cite{berger2013survey,dubinski.ea:2013:cloning,businge.ea:2018:appfamilies}. SPLE requires investment, such as training costs, organizational re-organizations, making assets not intended for reuse reusable (e.g., introducing configurable features), and creating model-based representations of the platform, typically as a feature model.



\looseness=-1
The following migration methods exist: Incremental migrations avoid disruptions, but the existing techniques are mainly process descriptions (e.g., performed by individuals in meetings) to analyze the domain by modeling features\,\cite{Bayer:1999:TLA:318773.319262,kang.ea:1990:foda,Bockle:2002:AIP:645882.672249}. The need for recording provenance information about features is also not recognized early during \co, before a platform is adopted. In so-called ``Big bang'' efforts, legacy systems are manually transformed into a product line and partially reimplemented. Such a process significantly impacts an organization's operation and immediate ability to develop new variants~\cite{Stallinger:2011:MTE:1985484.1985490}. Most of these frameworks are based on clone-detection techniques \cite{Faust:Verhoef:2003,Mende:Beckwermert:Koschke:Meier:2008,Mende:Koschke:Beckwermert:2009,Frenzel:Koschke:Breu:Angstmann:2007}, on data-mining techniques~\cite{Jiang:Zhang:Zhao:Zhou:2008}, on analyzing the history\,\cite{Yoshimura:Narisawa:Hashimoto:Kikuno:2008}, or other formal methods\,\cite{ryssel.ea:2010:AVI,rubin.ea:2012:transition}.
Still, such a migration of similar products into an integrated platform is expensive and risky, often leading to re-engineering efforts over years, as reported in industrial case studies~\cite{Jepsen:2007:MIM:1308171.1308202}.
Once we have features, evolving and maintaining features requires knowing the feature location in assets. 





}

\subsection{Clone Management and Variant Integration}\label{sec:clonemgmt}
\tb{TODO: significantly shorten this subsection; the next one on common activities is more important}
In what follows, we discuss five previous works on clone management and variant integration, which informed the design of the framework proposed in this paper.

\looseness=-1
\myparhead{Rubin \textit{et al.}\,\cite{rubin.ea:2013:framework,Rubin2015}} propose an abstract variant-integration framework, specifically a set of operators that a realization of such a framework should realize. The operators are derived from three case studies of organizations migrating cloned variants into a platform.



They propose a set of operators that extract feature-oriented information from design documents and code, and then link that information to code assets (feature location). They also define operators to mine information about feature dependencies and similarities---all typically require complex algorithms. After extracting this data, they reorganize the variants into clusters of related assets. Lastly, they compose various assets that result in a tentative architecture and a feature model. The application of the framework is discussed for the three case studies.
\longv{ 
}Notably, the framework supports the narrative that an operator-based perspective leads to more efficient implementation and support. However, their framework is much more abstract; our method and tool can be seen as a realization, relying on recording and exploiting meta-data. \longv{Consider their operator \textsf{findFeatures}, which is described as an operator that identifies features from assets, which usually requires expensive and inaccurate feature-location effort. In our case, we can easily retrieve this information from the asset tree (explained shortly, in \secref{sec:structures}). Furthermore, their work emphasizes the need to support different types of assets (code, requirements, design models, and tests), which we support with a programming-language-independent representation (the asset tree).}









\myparhead{ECCO} is a framework and tool, developed by Fischer \textit{et al.}\,\cite{fischer.ea:2014:ecco}, for composing new product variants using reusable artefacts (henceforth referred to as assets). The input to the framework is a set of variants realized via \co, each with a list of implemented features; additional cloned variants may be added over time. \textit{Extraction} is used to collect information about features and assets, as well as the feature interactions. \textit{Commonality analysis} on variants leads to a set of reusable assets along with dependencies between them. \textit{Composition} takes a selection of features and uses the reusable assets from extraction to compose a partial or complete product. \textit{Completion} guides the developers to fill in the missing implementation corresponding to features and feature interactions. The new variant is fed back into the system. \longv{
}
While the framework significantly improves reuse, maintaining the evolving assets and features might still impose some challenges. Even with the sophisticated techniques, the accuracy of the output is still affected by the lack of accuracy of feature location and clone detection.
\longv{We have the light-weight pairs of traces and mappings, for both features and assets, that support both reuse (via cloning) and maintenance (change propagation). Our active annotation strategy instead of passive extraction provides more flexibility in terms of feature model and asset tree related modifications and is more accurate because of the direct involvement of the developer during implementation. }

\myparhead{BUT4Reuse}, presented by Martinez \textit{et al.}\,\cite{MartinezBut4Reuse}, is an extraction-based technique for variant integration. The asset variants are used to build an asset model, and then the SPLE adopters (people relevant to the organization adopting SPLE) perform feature identification and feature location on the variants. Using the feature list and constraints, a feature model is synthesized. Lastly, using feature location traces, the reusable assets are created by extracting implementations of all features, and made suitable to be included in a product by composition. 
\longv{

}Since the goal is to facilitate the one-shot migration of a large set of variants towards a platform,
feature identification and location have to performed exhaustively.
Due to the lack of reliable automated techniques for the tasks, these are daunting and error-prone manual tasks, rendering the framework risk in practice.
Feature-to-code traceability is not recorded, as the scope of this framework is variant integration.



\myparhead{VariantSync}, developed by Pfofe \textit{et al.}\,\cite{variantsync:2016}, is a plugin-supported framework for automated synchronization of related software variants. Using FeatureIDE for feature model specification, it allows the developers to make changes to a program, and tag the code fragments to feature expressions. After a change, the developer can choose to perform a source- or target-focused change propagation. The former propagates the changes to all fragments whose tagged feature expression evaluates to true against the changed code's feature expression, whereas the latter only propagates changes to a specified code fragment. The merge conflicts arising during change propagation are resolved manually using java-diff-utils. 

The framework is light-weight and eliminates feature location. It also saves maintenance effort as the change propagation is automated. However, it is unclear how an asset can be reused automatically when a feature expression is tagged with it. Moreover, it is possible that a feature implementation is contained in an entire folder, or a set of files, instead of a few lines of code, whereas VariantSync primarily focuses on the code fragments.
\longv{Virtual Platform allows feature to asset mappings at any level in the repository (files, folders, code fragments), providing automated cloning (reuse) and change propagation (maintainence) for both features and assets.}

\myparhead{Montalvillo and D{\'\i}az}\,\cite{montalvillo2015tuning} propose supplementing Version Control Systems with operations that allow synchronization between artifacts belonging to the two distinct phases of SPLE: Domain Engineering and Application Engineering\,\cite{northrop2002software}. To this end, they specify a repository architecture comprising of a \textit{Core asset repository} and a set of \textit{product repositories}. On top of these, they define branching models that allow isolated development of core assets and customized products with two way propagations when needed. \textit{Update propagations} allow disseminating the changes in core assets to product repositories, while \textit{feedback propagations} feed changes introduced in product repositories back into the core assets repositories. Traditional VCS operations are used to provide these propagations, where development takes place in branches (\textit{branch, fork}) and product repositories use (\textit{clone}) assets from the core asset repository. Changes made to core assets or product-specific assets are propagated (\textit{merge}) when required.
\longv{
}To automate their approach, Montalvillo and D{\'\i}az\,\cite{montalvillo2015tuning} use web augmentation techniques to enhance Git with the proposed operations. The approach is novel and flexible, however it comes with the risk of the frequent need to resolve merge conflicts. Also, for a large number of products, the storage requirements inevitably grow and it can be difficult to keep track of which changes to propagate to which branch. Lastly, the need to locate feature will eventually rise and without a notion of \textit{features}, it will be difficult to trace which changes in implementation correspond to which features.







\subsection{Common Activities of Frameworks}\label{sec:clonemgmtactivities}

For a comparative analysis of the related frameworks, we extracted common activities performed by them.

The activities are performed in different ways and at different levels of automation.


\myparhead{Feature Identification} refers to the identification of the set of features implemented in a variant or a set of variants.
Different frameworks can have different mechanisms for feature identification, which may require additional artifacts as input (for example, requirements documents, or issue-tracker data).
They can also leave it to the user to specify the list of features, who can then decide to use an automated tool or perform the task manually.

\myparhead{Feature Location} involves recovering traceability between a feature of interest and related assets, in particular, the assets implementing the feature. A feature can be embedded in source code, mapped to a file or a folder, entailed in a requirements document.
When performed manually, feature location is an involved and error-prone tasks.
A great variety of automated techniques is available, all with different assumptions and capabilities; however, on realistic codebases, they usually either fall short in terms of precision or recall.


\myparhead{Feature Dependencies Management} supports maintenance of relationships between features, such as \textit{requires}, \textit{includes}, and \textit{is mutually exclusive with}. Since such relationships are common in product lines, the feature model notation allows specifying these relationships as well. Frameworks dealing with variant rich systems should include support for capturing and managing feature dependencies to manage complexity and prevent unwanted behavior. 

\myparhead{Feature Interactions Identification} refers to scenarios in which the selection of multiple features results in a behavior different to the behavior of the individual features. Feature interaction is an important aspect in software product lines, and an early identification of feature interactions can help prevent unexpected behaviors. 

\myparhead{Feature Model Creation} refers to the creation of a feature model, that is, a set of features in hierarchical structure along with their relationships and dependencies. Having a feature model offers a range of benefits; it captures the features, relationships between features and dependencies among features, thereby making it easier to check for valid and invalid configurations. Moreover, it is a non-technical asset which can act as a medium between different stakeholders.   


\myparhead{Storing Feature-to-Asset Mappings} refers to the maintenance of traceability links between the available features and the various assets in the project repository.
The availability of these links is crucial for clone management, to avoid that feature location has to performed repeatedly.

\myparhead{Clone Detection}, in our context, refers to the task of identifying cloned parts in a set of variants.
A well-established taxonomy \cite{roy2007survey} distinguishes four clones types, the first three of which are particularly relevant for our \co scenario:
\textit{identical parts}, \textit{almost-identical parts} (except for naming), \textit{similar parts} (identical modulo minor changes), and \textit{re-implementations} of the same functionality.
A large tool landscape of clone detectors is available and can support frameworks during clone management; however, these tools often have scalability vs. accuracy trade-offs.

\myparhead{Change Propagation} is the ability to automatically propagate changes (such as bug fixes, refactorings, and functionality additions) between variants.
When performed manually, change propagation involves a large effort to locate the targets of propagation (possibly in several variants), and replicate the changes made to the source variant.


\myparhead{Creation of Reusable Assets} refers to creation of assets that can later be used to derive variants, either directly or after some modification.
The reusable assets are usually equipped with a variability mechanism, that is, a mechanism for implementing variability in assets.
Compositional mechanisms, such as aspect-oriented programming, involve the splitting of assets in smaller building blocks; annotational mechanisms, such as preprocessor annotations, involved annotating the code with features \cite{kaestner.ea:2008:cide}.





\longv{\myparhead{Product Derivation} refers to the ability to derive a partial or complete product from a given configuration, that is, a valid selection of features.
A clone management framework may rely on the derivation method from the included variability mechanism:
In compositional mechanisms, assets are assembled from smaller building blocks; when using annotational mechanisms, certain annotated parts of an asset are removed to produce the assets of a variant \cite{kaestner.ea:2008:cide}.}


\myparhead{Variant Integration} is the merging of several variants while taking variability into account. When merging multiple versions of the same from two different variants, it is important to consider the features they map to.
Conflict arising during integration may be resolved manually or using automated tool support. This might require domain knowledge, and involve low-level code edits (for example adding preprocessor directives). 

\myparhead{Variant Comparison} is comparison of products with the intention of finding commonalities and variabilities. Similar to clone detection, variant comparison can be useful in feature identification, feature location, feature interactions identification.




In our framework, we used these activities as input to specify and formalize a suite of operators for seamless variant management.
Later in this paper, in \secref{sec:assessclonemgmt}, we elaborate on each considered framework's capabilities and user involvement when addressing these activities, thus supporting a comparative evaluation of our proposed framework.


\begin{figure}[t!]
	\centering
		\includegraphics[width=0.48\textwidth]{fig/overview.pdf}
	\caption{Overview (dashed boxes represent optional parts).}
	\label{fig:overview}
\end{figure}

\subsection{Other Related Works}\label{sec:plevolution}

Other works focus on problems arising once a product line has been migrated to product line platform.
For example, developers may want to perform changes that only affect dedicated products, without affecting other products. 
To this end, Neves \textit{et al.}\,\cite{neves2015safe} propose a set of operators for the \textit{safe evolution} of the product line. 
In contrast to our operationally defined operators, these operators are defined on an abstract level, based on their pre- and post-conditions; implementing them is left to the user.
\longv{Examples of these operators are \textit{add new optional feature}, \textit{split asset} or \textit{refine asset}. All operators operate on an abstract syntax tree, which, in our case, we generalize to a programming-language-independent asset tree (cf. \secref{sec:structures}).
Some of the patterns are synonymous to our operators, but work in a different context. For example, \textit{SplitAsset} is defined as extraction of the code fragment corresponding to a feature (made optional), and adding it to another asset (we have \textit{splitBlock} for annotating code fragments with features). 

The pre- and post conditions from their work can be incorporated into the Virtual Platform to further strengthen its well-formedness checks.}











Changes of the variability model may trigger corresponding changes of the implementation and vice versa, leading to a notion of co-evolution between both artifacts.
Based on a study of the Linux kernel, Passos \textit{et al.}\,\cite{passos.ea:2016:coevol} capture a set of evolution patterns.
Their variability model is defined in a feature-modeling-like language (Kconfig), which offers dedicated (domain-specific) modeling concepts for the Linux kernel. As such, their patterns specific to the Linux kernel.
\longv{For example, \textit{Add Computed Internal Non-Modular Feature} (ACINMF) refers to a feature representing a loadable kernel module, but whose value is derived from other features' values\,\cite{berger2013study}. However, we find patterns that are similar to those above, such as removing features, mapping assets to features, or splitting features.}


As a lightweight variability mechanism, Ji \textit{et al.}\,\cite{ji2015maintaining} present a system for annotating software assets with feature information. Specifically, feature locations are embedded directly into the assets and the project folder hierarchy, as well as a simple textual feature model \longv{(in Clafer syntax\,\cite{bak.ea:2010:sle,DBLP:journals/sosym/BakDACW16})}. They simulate the use of their annotation system on an open-source clone-based system, which we also adopt for our simulation (cf. \secref{sec:evaluation}).
\longv{Specifically, they identify 9 patterns with sub-patterns describing the evolution activities with respect to maintaining the feature annotations and exploiting them. Examples are: Adding or extending a feature, removing or disabling a feature or cloning a project. From that work, we got the inspiration that a flexible asset tree that carries feature information should be defined. Notably, some of our operators are more generic, for instance, their pattern cloning a project is represented by a generic asset clone operator in our case.}


==> tables/assetorientedfrequency.tex <==
\begin{table*}[t]
	\begin{tabular}{@{}llllll@{}}
		\toprule
		Operator                       & ClaferMooVisualizer & ClaferIDE & ClaferConfigurator & ClaferToolsUICommonPlatform & Total \\ \midrule
		\addasset       & 1027                & 183       & 711                & 1596                        & 3517  \\
		\changeasset    & 733                 & 229       & 176                & 68                          & 1206  \\
		\removeasset    & 801                 & 20        & 332                & 4                           & 1157  \\
		\cloneasset     & 25                  & 18        & 25                 & 9                           & 77    \\
		\propagateasset & 6                   & 2         & 4                  & 0                           & 12    \\ \bottomrule
	\end{tabular}
\end{table*}

==> tables/comparisonsmall.tex <==
\begin{table*}[t]
	
	
	\centering
	\caption{Virtual platform operators \tb{let's combine the columns input and output into 'signature' to save space (see my definitions in the operator section)}}\label{tab:operators}
	\vspace{-.3cm}
	\begin{adjustbox}{max width=\linewidth}
	
		\begin{threeparttable}
			\fontfamily{ptm}\selectfont
			\renewcommand{\arraystretch}{1}
			
			\begin{tabularx}{\textwidth}{
					l@{\hspace{1mm}}
					>{\hspace{1mm}}p{2.75cm}
					>{\raggedright\arraybackslash}p{3cm}
					
					>{\raggedright\arraybackslash}p{3cm}
					>{\raggedright\arraybackslash}p{7.3cm}
					c@{\hspace{.1em}}
				}
				
				\\
				& \textbf{\textsf{name}} & \textbf{\textsf{input}} & \textbf{\textsf{output}} & \textbf{\textsf{description}} \\ 
				
				
				
				\cmidrule[\heavyrulewidth]{2-5}
				
				\multirow{6}{1.5mm}[0mm]{\rotatebox{90}{\textbf{asset-oriented}}}

				&\addasset( S, T ) & Source Asset, Target Parent&Boolean verifier&The virtual platform checks for the well-formedness constraint between S and T, and if it is preserved, adds S to the list of sub-assets of the T. T is assigned as the parent of S. The global version number of the AST is incremented by one, and both S and T are assigned the global version. All other assets remain unchanged. All the features to which S maps to are added to the unassigned feature of the feature model relevant to T. Unassigned feature contains a list of all the features added as a result of asset addition. \\
				
				&\changeasset{T}&Target Asset&Boolean verifier&Change in T changes some attribute of T for example name or details. The global version number is incremented and the same version number is assigned to T. \\
				
				&\removeasset{R}{T}& AST Root, Target Asset	& Boolean verifier	& It is checked if the AST contains T. If it does, T is removed from the sub-asset's of it's parent. The parent of T gets the incremented global version. T is assigned a null parent. The global version number of the AST is updated. \\
				
				&\moveasset{S}{T}& Source Asset, New Target Parent	& Boolean verifier	& S is deleted from the sub-assets of it's parent. S is assigned the new parent T. S is added in the sub-assets of T. \wm{Haven't discussed the versioning protocol here. Should the global version number be acquired by both S and T?}\tb{fixed acc. to Wardah in the main text} \\
				
				&\addfeaturemodeltoasset{T}{FM} & Target Asset, Feature Model	& Boolean verifier	& FM is added as a feature model of T. The global version is incremented and assigned to T. \\
				
				&\mapassettofeature{T}{F} & Target Asset, Feature	& Boolean verifier	& F is added to the presence condition of T with a disjunction. The disjunction allows us to be not too conservative about the selection, such that if atleast one feature in the presence condition is selected, the asset is in the product configuration. Mapping an asset to a feature is essentially a change operation, and it follows the same versioning protocol. /the global version is incremented and assigned to T. Once an asset is assigned a feature model, all the assets below that asset can be mapped to any feature from the feature model.\\
				
				&\cloneasset{S}{T} & Source Asset, Target Parent	& Boolean verifier	& Cloning involves creating a deep clone of S and adding the clone (S*) to T. Every feature mapped to S is added in the incompleteimplementation feature of T's feature model. Incompleteimplementation feature holds a list of all features added to the feature model as a result of a clone operation. It is named so because it is possible that other assets from S*'s AST are mapped to it but they haven't been added. After feature cloning, new mappings between S* and the cloned features are created. The global version number is incremented and T gets the version number of the AST root. A new trace between the S and the S* is added to the trace database with the root's version number.\\
				
				&\propagateasset{S}{S*} & Source Asset, Source Clone	& Boolean verifier	& The trace database is traversed to verify that S* is a clone of S. If it is, then the version of S is compared against the version at which it was cloned. If S's version is ahead of that version, it is established that a change propagation is infact due. For propagation, S is deep-cloned (S**) and then all features mapped to S are cloned into the S*'s feature model if they are not already cloned. All the sub-assets of S* are added in S** if and only if they are consistent with or ahead of S. However if they are behind their respective source assets, the changes are recursively propagated until the complete S's subtree is traversed. New traces are created after every propagate operation. If there exists a sub-asset in the S, that is not cloned in the S*'s AST, it means it was added after the initial clone, and so it is cloned in S** retroactively. At the end, S** contains all the assets from S and S* at their latest updated state. S* is removed from the AST and S** takes its place. \\
				\cmidrule{2-5}
				
				\multirow{6}{1.5mm}[0mm]{\rotatebox{90}{\textbf{feature-oriented}}}
				& \addfeature{SF}{TF}{FM}& Source Feature, Target Feature, Feature Model & Boolean Verifier & If TF is provided, SF is added to the list of sub-features of TF. TF becomes the parent of SF. If TF is not given, SF is added as a top-level feature in FM. In both events, the global version of FM is updated. \\
				& \removefeature{FP} &  Feature Path & Boolean Verifier & FP is traversed to find the asset with the feature model (FM), and then FM is traversed to find the Target Feature TF. TF is deleted from it's parent feature if it is not a top-level feature. Otherwise it is deleted from the top-level features of FM. TF's parent is set to be null. All the assets previously mapped to TF are unmapped from TF. The assets only mapped to TF are removed after the removal of TF. FM's version number is updated. \\				
				& \makefeatureoptional{TF} & Target Feature & Boolean Verifier & TF's optional parameter is set to true, implying that it is no longer a mandatory feature.\wm{Versioning?} \\
				& \movefeature{SF}{TP}{FM} & Source Feature, Target Feature, Feature Model & Boolean Verifier & If both SF and TF belong to FM, SF is removed from the sub-features of it's parent, and added as a sub-feature of TF. SF's parent gets the value of TF.\wm{Versioning?} \\
				& \clonefeature{SFP}{TFP} & Source Feature Path, Target Feature Path & Boolean Verifier & Clone feature is also a deep clone operation. The source feature (SF) is extracted after traversing the feature path to find the asset with the source's feature model (SFM), and then finding SF in that. SF is cloned (SF*) and added to the TF's feature model (TFM). For all the assets mapped to SF, a tree slice is created, that has the dummy structure of the mapped asset upto the source asset containing SFM. This AST slice is a heirarchy of assets from the source asset down to the mapped asset, with only the details relevant for the mapped asset. The cloned asset is mapped to the SF* in accord with SF's mappings in source. The cloned asset's slice is added to the target asset. The global version TFM as well as the AST is incremented, and the newly added assets and their parents get the global version number. \\
				& \propagatefeature{SFP}{TFP} & Source Feature Path, Target Feature Path & Boolean Verifier &  Using SFP, The source's AST is traversed to find the asset containing the source feature model (SFM). Changes in the source feature including renaming, making optional and dependencies on any other feature are detected and propagated to the target feature (TF). All the assets mapped to SF, that are not cloned in the target AST are cloned in the target AST. New mappings between TF and the cloned assets are created. All the sub-features of SF, that are not cloned in the target's feature model (TFM) are cloned in TFM along with the assets that map to them. Propagation is a deep operation, meaning that it traverses all the subfeatures of SF until all the sub-features and relevant assets of TF are consistent with SF. \\			
				&	& & & \\
				
				
				\cmidrule[\heavyrulewidth]{2-5}
				
			\end{tabularx}
			\begin{tablenotes}[para]
				~\item[1] footnote 1...
			\end{tablenotes}
		\end{threeparttable}
		
	
	\end{adjustbox}
	
\end{table*}

==> tables/comparisontable.tex <==

\begin{table*}[ht]
	\fontsize{7}{7}\selectfont
	\centering
	\caption{Summary and comparison of state-of-the-art frameworks}\label{tab:comparisontable}
	\vspace{-.3cm}
	\begin{tabularx}{\linewidth}{P{1.5cm}P{2.4cm}P{2cm}P{2.4cm}P{2cm}P{2.4cm}P{2.4cm}}
		\toprule
		\textsf{\textbf{Activity}} & \textsf{\textbf{Rubin2015}} & \textsf{\textbf{ECCO}} & \textsf{\textbf{BUT4Reuse}} & \textsf{\textbf{VariantSync}} & \textsf{\textbf{Montalvillo \& D{\'\i}az}} & \textsf{\textbf{Virtual Platform}}\\
		\midrule
		
		
		\textbf{Feature Identification} & Abstract operator: findFeatures (Implementation not prescribed) & Activity: Features collected from user & Activity: Feature Identification (analysis and labeling of automatically generated blocks by domain experts) & Specified by developers in the beginning & Features not explicitly discussed & Specified by developers at any time using \addfeature\\
		
		
		\textbf{Feature Location} & Abstract operator: findFeatureImplementation (Implementation not prescribed) & Activity: Extraction (commonality analysis to identify feature implementation) & Activity: Feature location (automated block generation using variant comparison, Blocks labeled as features later by domain experts) & Changes in code tagged with feature expressions & Features not explicitly discussed & Specified by developer using \mapassettofeature\\
		
		\textbf{Feature Dependencies Management} & Abstract operator: dependsOn (mined from the project given two features from two variants, and a dependency type) & Not supported (asset dependencies are managed) & Activity: Constraint discovery (mine feature dependencies) & Specified by the developer in the beginning & Features not explicitly discussed & Specified during feature addition using \dependson  \\

		
		
		\textbf{Feature Model Creation} & Feature Model created using the result of findfeatures, dependsOn? Same? Interact? (discussed in the context of case studies) & Not supported & Activity: Feature Model Synthesis using constraint discovery (not supported but can be incorporated from literature) & Specified by the developer in the beginning & Features not explicitly discussed & Dynamically grows and shrinks with development \\
		
		
		
		\textbf{Mapping Assets to Features} & Abstract operator: findFeatureImplementation (Implementation not presribed) & Activity: Extraction (associations mined between features and assets given a set of variants) & Activity: Feature location (heuristic-based mapping given a feature list) & Feature expression-to-code mapping & Features not explicitly discussed & \mapassettofeature for mapping assets at any level in the AT\\
		
		\textbf{Clone Detection} & Textual diff-tools used (possible to add sophisticated clone detection techniques) & Added as future work & Not supported & Comparison of feature expressions for different assets & Artifacts cloned using \textit{Git clone}, point to the source artifact & Eliminated using \getclone\\
		
		\textbf{Feature Reuse by Cloning} & Not supported & Not supported & Not supported & Not supported & Features not explicitly discussed & \clonefeature\\
		
		\textbf{Change Propagation} & Activity: findfeatureimplementation to extract multiple implementations of one feature in different variants, same? for comparing them, propagating changes (implementation not prescribed) & Not supported & Not supported & Synchronization of variants by comparing feature expessions of changed fragment. & \textit{Update propagation} and \textit{feedback propagation} using \textit{Git merge} & \propagateasset, \propagatefeature \\
		
		\textbf{Creation of Reusable Assets} & Reusable components created incerementally by adding variants using operators merge and reorganize (Implementation not prescribed. discussed in case-study context) & Reuse associations between asset and features for composing new products & Activity: Reusable asset construction (Extract feature implementation using traceability information) & Not supported & \textit{Core assets} are reusable &  Assets and feature are reusable using \cloneasset and \clonefeature \\
		
		
		
		\textbf{Product Derivation} & Activity: Establish new variants, (clone the variant with most common functionality, remove extra features, add missing implementation (Implementation not prescribed) & Activity: Composition (Partial product composition against selected featured) & Composition of new product using reusable assets & Not supported & Cherry-picking \textit{core assets} and customizing them & Selection of features selects the code mapped to those to create a product \\
		
		\textbf{Integration} & Abstract operator: merge (Implementation not prescribed) & Not supported & Not supported & Manual conflict resolution after merging using java-diff-utils & Permanent changes merged from short-lived branches to long-lived branches & Conflicts resolved manually during change propagation \\
		
		\textbf{Variant Comparison} & Not supported & Comparison for feature location & Comparison for block identification & Not supported & \textit{Git diff} used to compare artifacts & Not required \\
		
		
		
		
		\bottomrule
	\end{tabularx}
	
	\begin{threeparttable}[b]
	\vspace{+.3cm}
		\begin{tabular}{ll}
			
			Not required & An activity or precessing step is not relevant in the framework, and has has no role in the contribution.\\
			Not supported & Activities and aspects that are relevant for the framework, and play a significant role in the contribution, but are missing, e.g., tool support.\\		
			Can be added & Enhancements that the authors imply can be added for better accuracy and performance, although not present in the framework.\\		
			Eliminated & Activities that would otherwise have to be undertaken but are eliminated due to the design and processing of the framework.\\		
			
		\end{tabular}
	\end{threeparttable}
	
	
\end{table*}



==> tables/costandbenefitcalculator.tex <==
\begin{table*}[t]
		\caption{Cost and benefit analysis of the ExpressionSolver toy example}
		\label{tab:costandbenefitcalculator}
		\begin{tabularx}{\columnwidth}{p{2cm}p{2cm}p{0.8cm}p{1.3cm}}
		\toprule
			\textsf{operator} & \textsf{BasicCalculator} & \textsf{Stack} & \textsf{ExpressionSolver}\\
			\midrule
			Number of assets					& 	7 & 2 & 2 \\
			Number of features				& 	10 & 2 & 2 \\
			Number of mappings 		 & 	7 & 2 &  2 \\
			Count of \cloneasset & 	7 & 2 &  0 \\
			Count of \clonefeature 				 & 	10 & 2 &  0 \\
			Asset Reuse 					& 	100\
			Feature Reuse 					& 	100\
			\propagateasset					&   3     &  0    &    0 \\
			\propagatefeature 				&   3     &  0    &    0 \\
			Number of feature locations eliminated		& 	13 & 2 &  0 \\	
			Number of clone detections eliminated   & 	3 & 0 &  0 \\
			\bottomrule					
		\end{tabularx}
\end{table*}




==> tables/helperfunctionstable.tex <==
\begin{table*}[t]
	\fontsize{7}{7}\selectfont
	\centering
	\caption{Helper functions}
	\vspace{-.3cm}
	\label{tab:helperfunctions}
	\begin{tabularx}{\linewidth}{p{3.5cm}p{13.5cm}}
		\toprule
		\textsf{function} & \textsf{description}\\
		\midrule
		\vpoperator{GetClones} & For a given asset or feature, traverse the trace database and return a list of all (clone) traces where the asset or feature is the source.
		\\
		\vpoperator{GetMappedFeatures}& For a given asset, return the list of features indicated by the presence condition.\\
		
		\vpoperator{GetMappedAssets}& For a given feature and AT (with any asset as root), return a list of all assets in the AT mapped to the feature. \\
		\vpoperator{AssetMappedToFeature}& For a given asset and feature, return true if the asset is mapped to the feature, otherwise false. \\
		\vpoperator{ASTContainsAsset}&For a given asset and AST, return true if the AT contains the asset, otherwise false. \\
		\vpoperator{FMContainsFeature}&For a given feature \vpsymbol{F} and feature model \vpsymbol{FM}, return true if \vpsymbol{FM} contains \vpsymbol{F}, otherwise false.\\
		\vpoperator{AssetCloned}& For a given asset \vpsymbol{A} and target parent asset \vpsymbol{T}, return true if a trace exists for \vpsymbol{A} and \vpsymbol{T}'s AT contains the clone of \vpsymbol{A}. \\
		\vpoperator{FeatureCloned}& For a given feature \vpsymbol{F} and target parent feature \vpsymbol{T}, return true if a trace exists for \vpsymbol{F} and \vpsymbol{T}'s AT contains the clone of \vpsymbol{F}. \\
		\vpoperator{GetAssetByName}&For a given asset name (or path) return the associated asset object. \\
		\vpoperator{GetLatestTrace}& For a given pair of source/target assets or features, return the most recent trace between them resulting from change propagation or cloning.\\
		\vpoperator{GetSlice} & For a given feature \vpsymbol{F}, cloning \vpsymbol{F} implies cloning all its mapped assets. This may involve obtaining slices of assets when some or all of the mapped assets are children of other assets that are not mapped to \vpsymbol{F}. For instance, if \vpsymbol{F} is mapped to class \vpsymbol{Add} in the file \vpsymbol{BasicCalculator/src/main/Add.java} (see \Figref{fig:getslice}), we would deep-clone the \vpsymbol{Add} class and clone all its ancestors without their children, up to the root folder: that is, \vpsymbol{Add.java} would only contain the \vpsymbol{Add} class (if more than one class exists), the folder \vpsymbol{main} would only have one file (\vpsymbol{Add.java}), and the \vpsymbol{src} folder would only have folder \vpsymbol{main}, etc.\\

		\bottomrule
	\end{tabularx}
\end{table*}

==> tables/operatorsrecognition.tex <==

\begin{table}[b]
	\caption{Recognition strategies for feature-oriented operators}
	\label{tab:operatorsrecognition}
\begin{tabular}{@{}ll@{}}
\toprule
Operator                               & Recognition Approach \\ \midrule
\addfeaturemodeltoasset & Automatic            \\
\addfeature             & Automatic            \\
\mapassettofeature      & Automatic            \\
\makefeatureoptional    & Semi-automatic       \\
\movefeature            & Automatic            \\
\removefeature          & Automatic            \\
\clonefeature           & Semi-automatic       \\
\propagatefeature       & Semi-automatic       \\ \bottomrule
\end{tabular}
\end{table}

==> tables/operatorstable.tex <==
\begin{table*}[t]
	
	
	\centering
	\caption{Virtual platform operators \tb{let's combine the columns input and output into 'signature' to save space (see my definitions in the operator section)}}\label{tab:operators}
	\vspace{-.3cm}
	\begin{adjustbox}{max width=\linewidth}
	
		\begin{threeparttable}
			\fontfamily{ptm}\selectfont
			\renewcommand{\arraystretch}{1}
			
			\begin{tabularx}{\textwidth}{
					l@{\hspace{1mm}}
					>{\hspace{1mm}}p{2.75cm}
					>{\raggedright\arraybackslash}p{3cm}
					
					>{\raggedright\arraybackslash}p{3cm}
					>{\raggedright\arraybackslash}p{7.3cm}
					c@{\hspace{.1em}}
				}
				
				\\
				& \textbf{\textsf{name}} & \textbf{\textsf{input}} & \textbf{\textsf{output}} & \textbf{\textsf{description}} \\ 
				
				
				
				\cmidrule[\heavyrulewidth]{2-5}
				
				\multirow{6}{1.5mm}[0mm]{\rotatebox{90}{\textbf{asset-oriented}}}

				&\addasset( S, T ) & Source Asset, Target Parent&Boolean verifier&The virtual platform checks for the well-formedness constraint between S and T, and if it is preserved, adds S to the list of sub-assets of the T. T is assigned as the parent of S. The global version number of the AST is incremented by one, and both S and T are assigned the global version. All other assets remain unchanged. All the features to which S maps to are added to the unassigned feature of the feature model relevant to T. Unassigned feature contains a list of all the features added as a result of asset addition. \\
				
				&\changeasset{T}&Target Asset&Boolean verifier&Change in T changes some attribute of T for example name or details. The global version number is incremented and the same version number is assigned to T. \\
				
				&\removeasset{R}{T}& AST Root, Target Asset	& Boolean verifier	& It is checked if the AST contains T. If it does, T is removed from the sub-asset's of it's parent. The parent of T gets the incremented global version. T is assigned a null parent. The global version number of the AST is updated. \\
				
				&\moveasset{S}{T}& Source Asset, New Target Parent	& Boolean verifier	& S is deleted from the sub-assets of it's parent. S is assigned the new parent T. S is added in the sub-assets of T. \wm{Haven't discussed the versioning protocol here. Should the global version number be acquired by both S and T?}\tb{fixed acc. to Wardah in the main text} \\
				
				&\addfeaturemodeltoasset{T}{FM} & Target Asset, Feature Model	& Boolean verifier	& FM is added as a feature model of T. The global version is incremented and assigned to T. \\
				
				&\mapassettofeature{T}{F} & Target Asset, Feature	& Boolean verifier	& F is added to the presence condition of T with a disjunction. The disjunction allows us to be not too conservative about the selection, such that if atleast one feature in the presence condition is selected, the asset is in the product configuration. Mapping an asset to a feature is essentially a change operation, and it follows the same versioning protocol. /the global version is incremented and assigned to T. Once an asset is assigned a feature model, all the assets below that asset can be mapped to any feature from the feature model.\\
				
				&\cloneasset{S}{T} & Source Asset, Target Parent	& Boolean verifier	& Cloning involves creating a deep clone of S and adding the clone (S*) to T. Every feature mapped to S is added in the incompleteimplementation feature of T's feature model. Incompleteimplementation feature holds a list of all features added to the feature model as a result of a clone operation. It is named so because it is possible that other assets from S*'s AST are mapped to it but they haven't been added. After feature cloning, new mappings between S* and the cloned features are created. The global version number is incremented and T gets the version number of the AST root. A new trace between the S and the S* is added to the trace database with the root's version number.\\
				
				&\propagateasset{S}{S*} & Source Asset, Source Clone	& Boolean verifier	& The trace database is traversed to verify that S* is a clone of S. If it is, then the version of S is compared against the version at which it was cloned. If S's version is ahead of that version, it is established that a change propagation is infact due. For propagation, S is deep-cloned (S**) and then all features mapped to S are cloned into the S*'s feature model if they are not already cloned. All the sub-assets of S* are added in S** if and only if they are consistent with or ahead of S. However if they are behind their respective source assets, the changes are recursively propagated until the complete S's subtree is traversed. New traces are created after every propagate operation. If there exists a sub-asset in the S, that is not cloned in the S*'s AST, it means it was added after the initial clone, and so it is cloned in S** retroactively. At the end, S** contains all the assets from S and S* at their latest updated state. S* is removed from the AST and S** takes its place. \\
				\cmidrule{2-5}
				
				\multirow{6}{1.5mm}[0mm]{\rotatebox{90}{\textbf{feature-oriented}}}
				& \addfeature{SF}{TF}{FM}& Source Feature, Target Feature, Feature Model & Boolean Verifier & If TF is provided, SF is added to the list of sub-features of TF. TF becomes the parent of SF. If TF is not given, SF is added as a top-level feature in FM. In both events, the global version of FM is updated. \\
				& \removefeature{FP} &  Feature Path & Boolean Verifier & FP is traversed to find the asset with the feature model (FM), and then FM is traversed to find the Target Feature TF. TF is deleted from it's parent feature if it is not a top-level feature. Otherwise it is deleted from the top-level features of FM. TF's parent is set to be null. All the assets previously mapped to TF are unmapped from TF. The assets only mapped to TF are removed after the removal of TF. FM's version number is updated. \\				
				& \makefeatureoptional{TF} & Target Feature & Boolean Verifier & TF's optional parameter is set to true, implying that it is no longer a mandatory feature.\wm{Versioning?} \\
				& \movefeature{SF}{TP}{FM} & Source Feature, Target Feature, Feature Model & Boolean Verifier & If both SF and TF belong to FM, SF is removed from the sub-features of it's parent, and added as a sub-feature of TF. SF's parent gets the value of TF.\wm{Versioning?} \\
				& \clonefeature{SFP}{TFP} & Source Feature Path, Target Feature Path & Boolean Verifier & Clone feature is also a deep clone operation. The source feature (SF) is extracted after traversing the feature path to find the asset with the source's feature model (SFM), and then finding SF in that. SF is cloned (SF*) and added to the TF's feature model (TFM). For all the assets mapped to SF, a tree slice is created, that has the dummy structure of the mapped asset upto the source asset containing SFM. This AST slice is a heirarchy of assets from the source asset down to the mapped asset, with only the details relevant for the mapped asset. The cloned asset is mapped to the SF* in accord with SF's mappings in source. The cloned asset's slice is added to the target asset. The global version TFM as well as the AST is incremented, and the newly added assets and their parents get the global version number. \\
				& \propagatefeature{SFP}{TFP} & Source Feature Path, Target Feature Path & Boolean Verifier &  Using SFP, The source's AST is traversed to find the asset containing the source feature model (SFM). Changes in the source feature including renaming, making optional and dependencies on any other feature are detected and propagated to the target feature (TF). All the assets mapped to SF, that are not cloned in the target AST are cloned in the target AST. New mappings between TF and the cloned assets are created. All the sub-features of SF, that are not cloned in the target's feature model (TFM) are cloned in TFM along with the assets that map to them. Propagation is a deep operation, meaning that it traverses all the subfeatures of SF until all the sub-features and relevant assets of TF are consistent with SF. \\			
				&	& & & \\
				
				
				\cmidrule[\heavyrulewidth]{2-5}
				
			\end{tabularx}
			\begin{tablenotes}[para]
				~\item[1] footnote 1...
			\end{tablenotes}
		\end{threeparttable}
		
	
	\end{adjustbox}
	
\end{table*}
